State Preparation in Quantum Optics

In quantum information and communication, optical schemes provide simple and intuitive experimental implementations. Of particular importance is quantum state preparation. In this thesis, the creation of polarisation entanglement using a particular class of optical circuits is studied. I give a mathematical description of this class of circuits in terms of Hermite polynomials. In this context, single photon resolution and single photon sensitivity detectors are discussed and compared with detector cascading. In addition, I study applications of state preparation such as quantum teleportation and quantum lithography.

==> text/declaration.tex <==
% This is the declaration for PhD theses. It needs the epic.sty file in 
% the `usepackage' environment. 
% Written by Pieter Kok.


\chapter*{}

\thispagestyle{empty}

\noindent
{\sc declaration}\medskip

\noindent
This work has not previously been accepted in substance for any degree and 
is not being concurrently submitted in candidature for any degree.

\bigskip

\noindent
Signed \mbox{\dottedline{2}(5,0)(150,0)} \hfil (candidate)

\medskip

\noindent 
Date \dottedline{2}(5,0)(163,0)

\vskip 1cm

\noindent
{\sc statement 1}\medskip

\noindent
This thesis is the result of my own investigations, except where otherwise 
stated. Other sources are acknowledged by footnotes giving explicit references.
A bibliography is appended.

\bigskip

\noindent
Signed \mbox{\dottedline{2}(5,0)(150,0)} \hfil (candidate)

\medskip

\noindent 
Date \dottedline{2}(5,0)(163,0)

\vskip 1cm

\noindent
{\sc statement 2}\medskip

\noindent
I hereby give consent for my thesis, if accepted, to be available for 
photocopying and for inter-library loan, and for the title and summary to be made available to outside organisations.

\bigskip

\noindent
Signed \mbox{\dottedline{2}(5,0)(150,0)} \hfil (candidate)

\medskip

\noindent 
Date \dottedline{2}(5,0)(163,0)

\newpage
\thispagestyle{empty}
